Interpretable exact linear reductions via positivity

Kinetic models of biochemical systems used in the modern literature often contain hundreds or even thousands of variables. While these models are convenient for detailed simulations, their size is often an obstacle to deriving mechanistic insights. One way to address this issue is to perform an exact model reduction by finding a self-consistent lower-dimensional projection of the corresponding dynamical system. Recently, a new algorithm CLUE has been designed and implemented, which allows one to construct an exact linear reduction of the smallest possible dimension such that the fixed variables of interest are preserved. It turned out that allowing arbitrary linear combinations (as opposed to zero-one combinations used in the prior approaches) may yield a much smaller reduction. However, there was a drawback: some of the new variables did not have clear physical meaning, thus making the reduced model harder to interpret. We design and implement an algorithm that, given an exact linear reduction, re-parametrizes it by performing an invertible transformation of the new coordinates to improve the interpretability of the new variables. We apply our algorithm to three case studies and show that "uninterpretable" variables disappear entirely in all the case studies. The implementation of the algorithm and the files for the case studies are available at https://github.com/xjzhaang/LumpingPostiviser.

==> case_studies/fceri.tex <==
     \subsection{Fc$\epsilon$-RI signaling pathways}
    \label{subsec:fceri}
    
    \subsubsection{Setup.} 
    We consider a model for a different kind of multisite phosphorylation \cite{Faeder2003}, a model for the early events in the signaling pathway of the high-affinity IgE receptor (Fc$\epsilon$RI) in mast cells and basophils.
    
    The model details the rule-based interactions of Fc$\epsilon$RI receptor with a bivalent ligand (IgE dimer), the Src kinase Lyn, and the cytosolic protein tyrosine kinase Syk.
   The model is based on the following sequence of signaling events in Fc$\epsilon$RI \cite{Metzger2002,Nadler2001} (the reactions are nicely summarized on~\cite[Figure~2]{Faeder2003}):
    
    \begin{enumerate}
        \item  binding of IgE ligand and Fc$\epsilon$RI receptor which aggregates at the plasma membrane,
        \item transphosphorylation of tyrosine residues in the immunoreceptor tyrosine-based activation motifs (ITAMs) of the aggregated receptor by constitutively associated Lyn,
        \item recruitment of additional Lyn and Syk kinase to the phosphorylated ITAM sites,
        \item transphosphorylation of Syk by Lyn and Syk on its linker region and activation loop, respectively.
    \end{enumerate}

    For visualizing different chemical species occurring in the resulting reaction network, we adopt the original graphic representation~\cite[Figure~1]{Faeder2003}, which is summarized in Figure~\ref{fceri_setup}.  
    In total, there are $354$ species that can be divided into three groups: monomers, dimers, and non-receptor states (free ligand, free Lyn, and Syk in each of its four possible states of phosphorylation).
    
    \begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/fig3.eps}
    \caption{\small Molecular components and states of the Fc$\epsilon$RI signaling events model.\\
    a. The IgE dimer is a bivalent ligand. Fc$\epsilon$RI consists of $\alpha$, $\beta$, and $\gamma$ subunits. 
    %A notch on the kinase indicates an SH2 domain, and a bump represents an ITAM site.
    The Lyn kinase has an SH2 domain. The Syk kinase has an SH2 domain and two ITAM sites. Syk ITAM sites are distinguished by the method of phosphorylation: Lyn phosphorylates the linker region, and Syk phosphorylates the activation loop.\\
    b. The $\alpha$ subunit can be unbound or bound to a ligand. The $\beta$ subunit can be unphosphorylated or phosphorylated, with or without associated Lyn. The $\gamma$ dimer can be unphosphorylated or phosphorylated, and the phosphorylated form bind to Syk in any of the four states of phosphorylation.}
    \label{fceri_setup}
    \end{figure}
    
    \begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/fig4.eps}
    \caption{\small Examples of a monomer, a dimer, and the free components.}
    \label{fig7}
    \end{figure}	
    
    \vspace{-5mm}
    \subsubsection{Reductions by ERODE and CLUE.} 
    The reduction by ERODE~\cite{Cardelli2017} consists of $105$ macro-variables, where all the complexes with the same configuration except for the phosphorylation state of the Syk units are summed up in a single macro-variable.
    We will refer to these macro-variables as \emph{Syk-macro-variables}.
    
    The model has been reduced using CLUE in~\cite[Section~4.2]{Ovchinnikov2021} with the observable being the total concentration of the free Syk (in all the four phosphorylation states). 
    The reduced model had $69$ macro-variables, and $51$ of them were nontrivial.
    It has been observed in~\cite[Section~4.2]{Ovchinnikov2021} that some of these macro-variable carry a physical interpretation, but in some of them, negative elements were present, which hinder their physical intelligibility.
    
    \subsubsection{Our results.}
    We apply our algorithm to the reduced model.
    {\color{red}Among the new macro-variables, we have $51$ nontrivial macro-variables which is the same as for the CLUE reduction.}
    %The algorithm also provides $69$ new macro-variable, and $51$ of which are nontrivial. 
    More precisely, \ref{step:producing} produced $57$ nontrivial macro-variables, and this number has been reduced to $51$ when computing a linearly independent basis on~\ref{step:greedy}.
    The resulting macro-variable refine the reduction by ERODE mentioned above in the sense that our new macro-variable are the sums of the Syk-macro-variables with non-negative coefficients.
    Therefore, in our reduction, all the complexes differing only by the phosphorylation state of the Syk units are in the same macro-variable.
    For the \emph{monomers}, we obtain the same reduction: nontrivial macro-variable involving monomers are of the form described on Figure~\ref{fig:fceri_monomer}. 
    
    \begin{figure}[!ht]
    \includegraphics[width=\textwidth]{figures/fig5.eps}
    \centering
    \caption{The monomer macro-variables. In each of them, $\alpha$ and $\beta$ are fixed, and we sum over all the phosphorylation patterns of Syk.}
    \label{fig:fceri_monomer}
    \end{figure}	
    
    The macro-variable involving dimers are graphically described on Figure~\ref{fig:fceri_dimers}.
    First, one can see that they are indeed linear combinations of the Syk-macro-variables.
    Our interpretation of these new macro-variables is based on two observations about the set of the reactions in the original model~\cite[Figure~2]{Faeder2003}:
    \begin{description}
        \item[\textbf{(Obs. 1)}] For every reaction involving a dimer, only one of the receptors of the dimer is affected by the reaction.
        \item[\textbf{(Obs. 2)}] The $\gamma$-chain of the other (not affected) receptor is relevant only for the reactions of transphosphorylation of Syk.
    \end{description}
    Since the complexes with different phosphorylation patterns are grouped together in the Syk-macro-variables, the second observation implies that the transphosphorylation reactions do not affect the values of the Syk-macro-variables at all.
    Therefore, the first observation suggests considering macro-variables as sums over all the dimer configurations in which one receptor is fixed (up to the phosphorylation of Syk), and for the other receptor, all the possible variants of the $\gamma$-chain are considered.
    
    With this interpretation in mind, let us take a closer look at the Figure~\ref{fig:fceri_dimers}:
    \begin{itemize}
        \item Each of the variables as on Figure~\ref{fig:fceri_noSyk} is the sum over the configurations with the fixed left receptor not carrying Syk and the right receptor having each of the six possible $\gamma$-chains.
        If one of the complexes in the sum is fully symmetric, it appears with coefficient 2.
        \item Each of the variables as on Figure~\ref{fig:fceri_Syk} is a combination of complexes that have: the same $\beta$-chains and Syk on the left receptor, any phosphorylation pattern of the Syk on the left receptor, and any $\gamma$-chain on the right receptor.
        If the $\beta$-chains on the receptors are equal, the complexes with two Syk's (which are \emph{symmetric up to} Syk phosphorylation) appear with coefficient 2.
    \end{itemize}
    
    Note that the coefficients $2$ appearing in the presence of symmetry prevent ERODE~\cite{Cardelli2017} from finding this reduction.
    
    \begin{figure}[!htbp]
        
        \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{figures/fig6a.eps}
         \caption{No Syk on the left $\gamma$-chain, the right takes all the possible $\gamma$-configurations}
         \label{fig:fceri_noSyk}
        \end{subfigure}    
        
        \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{figures/fig6b.eps}
    \caption{Syk (with all possible phosphorylations) on the left $\gamma$-chain, the right takes all the possible $\gamma$-configurations. }
    \label{fig:fceri_Syk}
        \end{subfigure}
        
        \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{figures/fig6c.eps}
    \caption{An example configuration of $Y_3$ (b) with identical $\beta$-chains. A variable has coefficient~2 when Syk kinases are recruited on both receptors (regardless of Syk state).}
    \label{fig:fceri_Syk2}
        \end{subfigure}
        \caption{Macro-variables involving dimers}
        \label{fig:fceri_dimers}
    \end{figure}
    
    
    
    % \subsubsection{Syk aggregation on dimers.} macro-variable that represent the aggregation of Syk states on dimers can be classified in two types: structures without Syk kinase attached and structures with existing Syk kinase attached.
    
    % There are 32 macro-variable whose initial molecule structure is a dimer without the recruitment of Syk kinase. Their graphical representation is provided in Figure~\ref{fig6}. Initially, there are 4 and 8 possible configurations for the two receptors. Thus, we have 26 possible configurations for the first dimer molecule in the macro-variable. 6 of the 26 possible configurations can recruit Syk on either receptor, which lead to separate linear combination of their respective phosphorylation states that follow. Therefore in total, we have $20 + 2 \times 6 = 32$ macro-variable. Each reaction involving a dimer affects only one of the receptors, so the $\gamma$-chain on the other receptor can be in either phosphorylation state.
    
    % \begin{figure}[!ht]
    % \includegraphics[width=\textwidth]{figures/fig6.eps}
    % \caption{New macro-variable structure for the aggregation of Syk states on dimer configurations without Syk initially.}
    % \label{fig5}
    % \end{figure}
    
    % There remain 16 macro-variable whose initial molecule structures are dimers that have recruited a single Syk. There are $n_{\beta} = 4$ possible configurations for a receptor and 16 possible configurations for a dimer of the given form in Figure~\ref{fig7}. We observe the phosphorylation of the existing Syk kinase, then the recruitment and phosphorylation of a second Syk kinase. When a dimer has identical $\beta$-chain configurations on its receptors and has recruited two Syk kinases, the variable's coefficient is two. This can be explained from the perspective of our observable, which is the aggregation of all Syk phosphorylation patterns. The model does not distinguish the specific states of Syk phosphorylation and considers the dimer to be symmetric with respect to its receptors. Six of the macro-variable are omitted in the new reduced model due to linear dependence. We notice the complete preservation of physical structures by our method.
    
    % \begin{figure}[!ht]
    % \includegraphics[width=\textwidth]{figures/fig7.eps}
    % \caption{New macro-variable structure for the aggregation of Syk states on dimer configurations with Syk initially. If the dimer has recruited Syk kinases on both receptors, the variable has a coefficient two.}
    % \label{fig6}
    % \end{figure}	
    
    

==> case_studies/jak.tex <==
\subsection{Jak-family protein tyrosine kinase activation}
\label{subsec:barua}
\subsubsection{Setup.} 
We study a simplified cellular model of a bipolar ``clamp" mechanism for Jak-family kinase activation \cite{Barua2009}. 
Kinases of the Janus kinase (JAK) family play an essential role in signal transduction mediated by cell surface receptors, which lack innate enzymatic activities to dimerize. 
    
The model studies the interactions of Jak2 kinase trans-phosphorylation, specifically the rule-based dynamics between the Jak2 (J) kinase, the unique adaptor protein SH2-B$\beta$ (S) with the capacity to homo-dimerize, the growth hormone receptors (R), and a bivalent growth hormone ligand (L). The Jak2 kinase has two phosphorylation sites, Y1 and Y2. The SH2-B$\beta$ protein contains an N-terminal dimerization domain (DD) and a  C-terminal  Src homology-2  (SH2) domain. 

The components can interact in the following ways:
    \begin{enumerate}
        \item binding of ligand and growth hormone receptors which aggregates at the plasma membrane,
        \item constitutive binding of Jak2 kinase to the receptors, which autophosphorylates on the phosphorylation sites when two Jak2 kinases are bounded in the same complex,
        \item recruitment of SH2-B$\beta$ protein at the SH2 domain by the Jak2's autophosphorylated Y1 site,
        \item dimerization of SH2-B$\beta$ protein through recruitment of an additional SH2-B$\beta$ protein, engaged at the DD domains.
    \end{enumerate}

Receptors can undergo a process of \emph{internalization}, in which the receptors can no longer associate with any Jak2, and the existing Jak2 and SH2-B$\beta$ in the complex can dissociate at the normal rate. 
  \begin{figure}[!htbp]
     \centering
    \includegraphics[width=.9\textwidth]{figures/fig7.eps}
    \caption{\small Components of the Jak-family protein tyrosine kinase activation model.\\}
    \label{barua_setup}
    \end{figure}

\subsubsection{Reductions by ERODE and CLUE.}
The reduction obtained by ERODE in~\cite[Figure~5]{Cardelli2017} contained $345$ macro-variables. 
It grouped the internalized configurations, which differ by the connections between the receptors and the ligand, into macro-variables.

The model has been reduced by CLUE in~\cite{Ovchinnikov2021}, with the observable being the concentration of the free ligand. 
The reduced model had $322$ macro-variables, and $69$ of them were nontrivial.
The model has been used in~\cite{Ovchinnikov2021} for benchmarking purposes only, so the macro-variables have not been interpreted.
The reduction included several macro-variables with negative coefficients, including one with 20 nonzero coefficients.
We do not see any natural interpretation for them.

\subsubsection{Our results.}  
We apply our algorithm to the reduced model, 
%which provides $322$ macro-variables and $70$ nontrivial macro-variables during~\ref{step:producing}, which is reduced to $69$ when computing a linearly independent basis on~\ref{step:greedy}. 
{\color{red}and among the produced macro-variables $69$ are nontrivial as in the reduction by CLUE (\ref{step:producing} produces $70$ macro-variables, and then this number is reduced to $69$ at~\ref{step:greedy}).}
The nontrivial macro-variables are linear combinations of internalized molecules, and the trivial macro-variables are not internalized. 
Compared to the ERODE reduction, some internalized complexes such as the ligand-receptor (R, RL, RLR) structures in \cite[Figure~5(C)]{Cardelli2017}, are omitted in our model as they do not disassociate under internalization and thus do not affect the dynamics of the free ligand observable. 
In our reduction, mirrored internalized complexes are lumped together, which explains all two-element macro-variables.
The remaining nontrivial macro-variables are described on Figure~\ref{fig:barua}, and are of two types:
\begin{itemize}
    \item \emph{Configurations equivalent up to the connection between the ligand and the receptors (Figure~\ref{fig:barua}-a and~\ref{barua_fig2}).}
    The structures are equivalent under internalization as the ligand and receptors cannot disassociate and were obtained also by ERODE~\cite[Figure~5(D, E)]{Cardelli2017}. 
    They are of two types: single-Jak2-Receptor case (Figure~\ref{fig:barua}-a) and ``clamp'' case (Figure~\ref{barua_fig2}).

    
    \item \emph{Configurations with one receptor fixed (Figure~\ref{fig:barua}-b).}
    These are similar to Figure~\ref{fig:fceri_dimers} from the case study in Section~\ref{subsec:fceri}:
    since in the reactions with internalized complexes, only one receptor is affected, and this does not depend on the state of the other receptor, one can group together the complexes having one of the receptors the same.

    When the receptors are symmetric, the element and its mirrored element are the same, so the corresponding configuration appears with coefficient~2.
\end{itemize}

  \begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/fig8.eps}
    \caption{\small Classes of internalized macro-variables.
    a. equivalent up to the connection between the ligand and the receptors.
    b. one receptor fixed.}
    \label{fig:barua}
    \end{figure}
  \begin{figure}[!htbp]

    \includegraphics[width=\textwidth]{figures/fig9.eps}
    \caption{\small Macro-variables for equivalent structures of the bipolar "clamp" mechanism}
    \label{barua_fig2}
    \end{figure}
    
        % The macro-variables representing the aggregation of SH2-B$\beta$ molecules are given in Figure \ref{fig:barua}-b. We observe that one receptor of the complex recruits SH2-B$\beta$ molecules, which is possible under internalization and the fact that the associated reactions only affect one receptor. 
            % Three macro-variables represent the equivalent structures associated with the bipolar "clamp" mechanism (RJS$_2$JR), which is detailed in Figure \ref{barua_fig2}.

==> case_studies/mphos.tex <==
    \subsection{Multisite protein phosphorylation}
    \label{subsec:case1}
    
	\subsubsection{Setup.} We consider a model of multisite phosphorylation \cite{Sneddon2010}.
	%which has also been considered in the original CLUE paper~\cite[Section~4.2]{Ovchinnikov2021}.
	It describes a protein with $m$ identical and independent binding sites that simultaneously undergo phosphorylation and dephosphorylation.
	Each binding site can be in one of the four different states (see Figure~\ref{fig:multisite_setup}):
	\begin{enumerate}
	    \item unphosphorylated and unbound, 
	    \item unphosphorylated and bound to a kinase,
	    \item phosphorylated and unbound,
	    \item phosphorylated and bound to a phosphatase.
	\end{enumerate}
    Therefore, there are $4^m + 2$ chemical species in the corresponding reaction network: free kinase and phosphatase, and $4^m$ states of the protein.
    
    \subsubsection{Reductions by ERODE and CLUE.} 
    In the reduction computed by ERODE~\cite{Cardelli2017} (for $m = 2, \ldots, 8$), the concentrations of protein configurations are replaced by the sums of the concentrations of configurations differing by a permutation of the sites.
    Therefore, the number of macro-variables is equal to $\binom{m + 3}{3} + 2$.
    
    In contrast, the analysis performed by CLUE~\cite{Ovchinnikov2021} always results in just six macro-variables.
    Two of them were always the concentrations of kinase and phosphatase as for ERODE.
    The other four were linear combinations with protein configurations.
    In~\cite[Section 4.2]{Ovchinnikov2021}, for $m = 2$, interpretation was provided for the first three of them. However, for the last one, it was remarked that ``the last macro-variable escaped physical intelligibility as it represents the difference between the free substrate with unphosphorylated sites and protein configurations that appear in the aforementioned lumps."
    
    
	\begin{figure}[!htbp]
	\centering
    \includegraphics[width=0.9\textwidth]{figures/fig1.eps}
    \caption{\small Molecular components and states of the multisite phosphorylation model. \\
    a. Consists of multisite proteins and kinases. This example has $m = 3$ phosphorylation/binding sites.\\
    b. There are 4 possible states for a single binding site: unphosphorylated and unbound, unphosphorylated and bound to a kinase, phosphorylated and unbound, phosphorylated and bound to a phosphatase.}
    \label{fig:multisite_setup}
    \end{figure}
    
    \subsubsection{Our results.} We applied our algorithm to the cases $m = 2, 3, 4, 5$ and obtained new macro-variables, which have again included the concentrations of free kinase and phosphatase.
    Moreover, the three interpretable macro-variables from the analysis in~\cite{Ovchinnikov2021} for $m = 2$ are kept.
    Each of the four our macro-variables involving the protein configurations corresponds to a state of a site (e.g., unbounded and unphosphorylated), and each protein configuration appears with a coefficient equal to the number of sites in it with this state.
    Examples of these new macro-variables are given on Figure~\ref{fig:multisite_example} for $m = 2$ and $m = 3$.
    
    One way to interpret the result is that the constructed reduction replaces the concentration of the protein configurations with the ``concentrations'' of each of the four states of the sites (see also Example~\ref{ex:lumping}).
    From our interpretation, we expect that the models with larger $m$ will have a reduction of the same form.
    
    
    \begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/fig2.eps}
    \caption{\small New macro-variables for $m = 2, 3$. 
    Each state of a binding site from Fig~\ref{fig:multisite_setup}-b can be the main state, yielding four macro-variables for each $m$. 
    The coefficients are equal to the number of binding sites in a protein that are in the main state.}
    \label{fig:multisite_example}
    \end{figure}

    % Through our algorithm, we provide a reduced model with four new macro-variables. Examples of their configurations are provided in Figure~\ref{fig2}, where we give the graphical representations for the first macro-variable in models with $m=2$ and $m=3$ phosphorylation sites. In both cases, the remaining three macro-variables follow the same form as the first, with their main states being the other three possible states of a binding site. In every macro-variable, the coefficient of a variable (protein configuration) is equal to the number of binding sites it has in the main state.
    
    % From the observed aggregation, we suggest the four new macro-variables represent the total concentrations of the four possible binding site configurations.
    

==> introduction/abstract.tex <==
Kinetic models of biochemical systems used in the modern literature often contain hundreds or even thousands of variables.
While these models are convenient for detailed simulations, their size is often an obstacle to deriving mechanistic insights.
One way to address this issue is to perform an exact model reduction by finding a self-consistent lower-dimensional projection of the corresponding dynamical system.


Recently, a new algorithm CLUE~\cite{Ovchinnikov2021} has been designed and implemented, which allows one to construct an exact linear reduction of the smallest possible dimension such that the fixed variables of interest are preserved.
It turned out that allowing arbitrary linear combinations (as opposed to zero-one combinations used in the prior approaches) may yield a much smaller reduction.
However, there was a drawback: some of the new variables did not have clear physical meaning, thus making the reduced model harder to interpret.

We design and implement an algorithm that, given an exact linear reduction, re-parametrizes it by performing an invertible transformation of the new coordinates to improve the interpretability of the new variables.
We apply our algorithm to three case studies and show that ``uninterpretable'' variables disappear entirely in all the case studies.
	    
The implementation of the algorithm and the files for the case studies are available at \url{https://github.com/xjzhaang/LumpingPostiviser}.

% Such exact reductions may be further combined with approximation-based order reduction techniques.

==> introduction/intro.tex <==
Dynamical models described by systems of polynomial ordinary differential equations (PODEs) are frequently used in systems biology and life sciences in general.
One of the major classes of such models is the dynamical models of chemical reaction networks (CRN) under the mass-action kinetics in which each indeterminate corresponds to the concentration of one of the chemical species.
Models appearing in the literature often consist of hundreds or thousands of variables.
While the models of this size can incorporate a substantial amount of information about the phenomena of interest, it is often hard to use them to derive mechanistic insights.

One way to address these challenges is to use \emph{model reduction} algorithms that replace a model with a simpler one while preserving, at least approximately, some of the features of the original model.
A wide range of methods has been developed for approximate model reduction, including methods based on singular value decomposition~\cite{antoulas} and time-scale separation~\cite{okino1998}.

A complementary approach is to perform~\emph{exact model reduction}, that is, lower the dimension of the model without introducing approximation errors.
For example, exact linear lumping aims at writing a self-consistent system of differential equations for a set of \emph{macro-variables} in which each macro-variable is a linear combination of the original variables.
For important classes of biochemical models, specialized lumping criteria have been developed (see, e.g., ~\cite{Borisov,Conzelmann,Feret}), allowing the construction of macro-variables as sums of some of the original variables (that is, allowing only coefficients zero and one in the linear combinations).
A general lumping algorithm has been proposed in~\cite{Cardelli2017,erode} which is applicable to any system of PODEs (not necessarily arising from a CRN).
This algorithm partitions the original variables so that the macro-variables can be the sums of the variables within the blocks in the partition.
Note that the macro-variables are zero-one linear combinations of the original variables in all these cases.

In~\cite{Ovchinnikov2021}, an algorithm has been designed (and the corresponding software called \emph{CLUE} presented) that, for a given set of linear forms in the state variables (the \emph{observables}), constructs a linear lumping of the smallest possible dimension such that the observables can be written as combinations of the macro-variables (i.e., the observables are preserved).
Unlike the earlier approaches, the macro-variables produced by CLUE may involve any coefficients, and this allowed to produce reductions of lower dimensions than it was possible before, see~\cite[Table~1]{Ovchinnikov2021}.
However, there was a price to pay for this flexibility: the authors state that some of the produced macro-variables ``escape physical intelligibility'' (see~\cite[Section~4.2]{Ovchinnikov2021}).
Indeed, the resulting reduction of the smallest dimension is uniquely defined up to a linear change of the coordinates, so the coordinates in the reduced state space chosen by CLUE could be not optimal in the sense of interpretability.

In this paper, we propose a post-processing step that takes an exact linear lumping (not necessarily produced by CLUE) and attempts to improve its interpretability by performing a change of variables.
It has been observed in~\cite{Ovchinnikov2021} that one of the sources of difficulties for interpretation is the negative coefficients in the macro-variables.
We design and implement an algorithm that finds (if possible) a linear change of variables in the reduced model so that
\begin{enumerate}
  \item the coefficients of the representations of the new macro-variables in terms of the original state variables are nonnegative

  \item and the total number of nonzero coefficients in these representations is as small as possible.
\end{enumerate}
We demonstrate the efficiency of our approach on three case studies from the literature.
Two of these cases are exactly the case studies from~\cite{Ovchinnikov2021} in which issues with interpretability occur.
We show that our method provides interpretable re-parametrizations of the optimal lumpings computed by CLUE in all three case studies.
Our algorithm uses tools from convex discrete geometry and matroid theory.
%     Dynamic models of biochemical systems carry valuable information about the complex interactions between different components of the studied systems. They are essential for understanding the mechanisms of the underlying systems and predicting the behaviors of a biological process under different circumstances. For models to be accurate, in systems biology, mechanistic models are constructed by series of ordinary differential equations (ODEs) combined with the law of mass action that detail the specific interactions between different components of the system. As molecules in biological systems tend to interact with one another in distinct combinations, the models are oftentimes combinatorially complex \cite{Sneddon2010}.  In consequence, it is challenging to derive physical interpretations from them. 
	
% 	Model reduction methods are designed to reduce the complexity of dynamic models by providing reduced models of lower-dimensionality that preserve the same dynamical features as the original model. In systems biology, this simplification is beneficial as it allows researchers to work with less-complex models with reduced kinetic parameters that are still accurate representations of the systems \cite{Dan2006}. However, in many model reduction methods, the original structure of the model is often destroyed in the process, which leads to a loss of underlying physical meaning that is valuable to models of systems biology \cite{Apri2012,Schmidt2008,Sunnker2011}.
	
% 	To approach this problem, some model reduction algorithms are created with the notion of maintaining physical intelligibility. 
% 	CLUE, an algorithm for exact model reduction, performs exact linear lumping that, to some degree, protect the physical structure of the original model. 
% 	Nevertheless, despite preserving the physical structure, the reduced models of CLUE remain, at times, limited in physical interpretability.
	
% 	In this paper, we propose a method to re-represent reduced models from CLUE with overall improved physical intelligibility.
